Development and Validation of Functional Model of a Cruise Control System

Modern automobiles can be considered as a collection of many subsystems working with each other to realize safe transportation of the occupants. Innovative technologies that make transportation easier are increasingly incorporated into the automobile in the form of functionalities. These new functionalities in turn increase the complexity of the system framework present and traceability is lost or becomes very tricky in the process. This hugely impacts the development phase of an automobile, in which, the safety and reliability of the automobile design should be ensured. Hence, there is a need to ensure operational safety of the vehicles while adding new functionalities to the vehicle. To address this issue, functional models of such systems are created and analysed. The main purpose of developing a functional model is to improve the traceability and reusability of a system which reduces development time and cost. Operational safety of the system is ensured by analysing the system with respect to random and systematic failures and including safety mechanism to prevent such failures. This paper discusses the development and validation of a functional model of a conventional cruise control system in a passenger vehicle based on the ISO 26262 Road Vehicles - Functional Safety standard. A methodology for creating functional architectures and an architecture of a cruise control system developed using the methodology are presented.

==> eptcsdata.tex <==
\providecommand{\firstpage}{45}
\providecommand{\publicationstatus}{J. Kofro\v{n}, J. Tumova, B. Buhnova (Eds.): Formal Engineering\\
Approaches to Software Components and Architectures (FESCA'16)\\
EPTCS 205, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.205.4}{10.4204/EPTCS.205.4}}
\pdfoutput=1

